A Scalable Near-Memory Architecture for Training Deep Neural Networks on Large In-Memory Datasets

Most investigations into near-memory hardware accelerators for deep neural networks have primarily focused on inference, while the potential of accelerating training has received relatively little attention so far. Based on an in-depth analysis of the key computational patterns in state-of-the-art gradient-based training methods, we propose an efficient near-memory acceleration engine called NTX that can be used to train state-of-the-art deep convolutional neural networks at scale. Our main contributions are: (i) a loose coupling of RISC-V cores and NTX co-processors reducing offloading overhead by 7x over previously published results; (ii) an optimized IEEE754 compliant data path for fast high-precision convolutions and gradient propagation; (iii) evaluation of near-memory computing with NTX embedded into residual area on the Logic Base die of a Hybrid Memory Cube; and (iv) a scaling analysis to meshes of HMCs in a data center scenario. We demonstrate a 2.7x energy efficiency improvement of NTX over contemporary GPUs at 4.4x less silicon area, and a compute performance of 1.2 Tflop/s for training large state-of-the-art networks with full floating-point precision. At the data center scale, a mesh of NTX achieves above 95% parallel and energy efficiency, while providing 2.1x energy savings or 3.1x performance improvement over a GPU-based system.

==> sec_compat.tex <==
% ==============================================================================
\section{Computational Patterns}
\label{sec:compat}



% ------------------------------------------------------------------------------
\subsection{Stochastic Gradient Descent}
\label{sec:compat:sgd}

\gls{sgd} is the most used optimization algorithms for machine learning \cite{Goodfellow2016}. Given a neural network $f(x;\theta)$, it optimizes the network parameters $\theta$ to minimize a loss function $L(f(x;\theta),\hat y)$. This function models the deviation of the actual output $f(x;\theta)$ from the desired output $\hat y$. In its simplest form, \gls{sgd} consists of evaluating the loss function for different inputs $x$ (\emph{forward pass}, \eqnref{eq:fwdpass}), finding the derivative with respect to $\theta$ (\emph{backward pass}, \eqnref{eq:bwdpass}), and then updating the network parameters (\eqnref{eq:wupd}). In practice the learning rate $\epsilon$ is being varied as training progresses.
%
\begin{align}
l_i(\theta) &= L(f(x_i;\theta),\hat y_i)  \label{eq:fwdpass} \\
g &= \frac{1}{m} \nabla_\theta \sum_{i=1}^m l_i  \label{eq:bwdpass} \\
\theta &\leftarrow \theta - \epsilon g  \label{eq:wupd}
\end{align}
%
where $m$ is the number of inputs $x_i$ (\emph{batch size}) and $\hat y_i$ is the desired output for input $x_i$. Besides the forward and backward pass, \gls{sgd} only requires support for the WAXPBY (scaled vector addition, \eqnref{eq:wupd}) operation in order to perform a full training step on an accelerator.

\subsubsection{Momentum}
\label{sec:compat:sgd:momentum}

A common extension to \gls{sgd} is the concept of momentum \cite{polyak1964some}, which introduces a ``velocity'' $v$ that is carried over from one training step to the next. Rather than directly affecting the parameters as in \eqnref{eq:wupd}, the gradient is now used to alter the velocity which in turn is used to update the parameters:
%
\begin{align}
v &\leftarrow \alpha v - \epsilon g  \label{eq:wupd:mom} \\
\theta &\leftarrow \theta + v
\end{align}
%
A further variation on this concept \cite{sutskever2013importance} introduces an additional interim update to the parameters before the gradient is calculated. The fundamental operation of the weight update remains WAXPBY.

\subsubsection{AdaGrad, RMSProp, and Adam}
\label{sec:compat:sgd:adagrad}
\label{sec:compat:sgd:rmsprop}

The AdaGrad \cite{duchi2011adaptive} and RMSProp \cite{tieleman2012lecture} variations on \gls{sgd} use an adaptive learning rate. In both cases the squared gradient is accumulated across iterations and used to adjust the learning rate as training progresses. The weight update for RMSProp looks as follows:
%
\begin{align}
r &\leftarrow \rho r + (1-\rho) g \odot g \\
\theta &\leftarrow \theta - \frac{\epsilon}{\sqrt{\delta + r}} \odot g
\end{align}
%
Note that the multiplication $\odot$, division, and square-root operations are applied element-wise. In this case an accelerator must also support vector multiplication, division, and square-root operations to perform a full training step.

The Adam algorithm \cite{Kingma2014} keeps separate track of first and second moments across iterations to adaptively adjust the learning process, but uses the same set of fundamental operations.



% ------------------------------------------------------------------------------
\subsection{Layer Diversity}
\label{sec:compat:layers}

\input{tables/compat_layers}

Contemporary \glspl{dnn} consist of a variety of different layers. \tabref{tbl:compat:layers} provides an overview of the layers used in the \glspl{dnn} considered in this work. We observe that the layers making up the bulk of computation, namely convolutions and linear layers \cite{azarkhish2017neurostream, Goodfellow2016, venkataramani2017scaledeep}, boil down to \gls{mac} reduction operations \cite{Abadi2016, jia2014caffe, collobert2008torch}. Non-linear operations such as max pool and \gls{relu} require additional comparison operations. All other layers can be distilled into vector addition and multiplication operations, either due to their nature or by approximating them iteratively. An iterative approach is feasible if the approximated function is used rarely within the overall computation, which is often the case for div, exp, log, sqrt, and others. We thus conclude that an arithmetic unit capable of vectorized MAC and comparison operations is sufficient to efficiently perform the computations that arise in the considered \glspl{dnn} (\tabref{tbl:compat:layers}). Note that while inference architectures also support these operations, other concerns such as data scheduling and the availability of memory prevent their use for training.



% ------------------------------------------------------------------------------
\subsection{Inference vs.\@ Training}
\label{sec:compat:infvstrain}

The computations involved in applying a neural network to an input can be described as a \gls{dag}, see \figref{fig:intro:flow}. The layered nature of this graph makes the represented computation amenable to hardware acceleration: The operations can be performed layer-by-layer, requiring only a limited amount of memory to carry intermediate results from one layer to the next.

The training of such networks on the other hand requires various derivatives to be computed. Given a computation graph that describes the network (forward pass), automatic differentiation \cite{rall1981automatic} may be used to find a complementary graph (backward pass) that determines the parameter derivatives. The added operations introduce unfavorable dependencies on the intermediate results of the forward pass: The very last derivative to be computed depends on the very first intermediate result produced, thus requiring significantly more memory than the forward pass, where intermediate results could just be discarded.

Consider the convolutions of ResNet-34 listed in \tabref{tbl:compat:tmpmem} for example. For an inference step, the layer with the largest output size dictates the amount of memory required, i.e. $803\cdot 10^3$ values. For a training step, the output of each layer must be kept in memory, i.e. $3560\cdot 10^3$ values.

\begin{table}
% \begin{threeparttable}
\caption{Intermediate result sizes of the convolutions in ResNet-34. Note that layers are repeated multiple times. During inference, the memory must hold the largest intermediate result, i.e. the $max(\cdot)$ of all output sizes. During training, it must hold all intermediate results, i.e. the $\sum\cdot$ of all output sizes and repetitions.}
\label{tbl:compat:tmpmem}
\vspace{-1.5em}
\center
\begin{tabular}{@{}lll k{7} k{7}@{}}
	\toprule
	{\bfseries Layer} &
	{\bfseries Rep.} &
	{\bfseries Output Size} &
	{\bfseries Inference} &
	{\bfseries Training} \\
	% & {$r$} & {$d$} & {$\max d$} & {$\sum r d$} \\
	\midrule
	conv1 & $ 1\times$ & $112\cdot112\cdot 64$ & 803000 &  803000 \\
	conv2 & $ 6\times$ & $ 56\cdot 56\cdot 64$ & 201000 & 1200000 \\
	conv3 & $ 8\times$ & $ 28\cdot 28\cdot128$ & 100000 &  802000 \\
	conv4 & $12\times$ & $ 14\cdot 14\cdot256$ &  50200 &  602000 \\
	conv5 & $ 6\times$ & $  7\cdot  7\cdot512$ &  25100 &  151000 \\
	\midrule
	&&& 803000 & 3560000 \\
	\bottomrule
\end{tabular}
% \end{threeparttable}
\end{table}



% ------------------------------------------------------------------------------
\subsection{Convolutional Neural Networks}
\label{sec:compat:cnn}

\subsubsection{Convolution Shapes}
\label{sec:compat:cnn:shape}

Convolution operations are abundant in \glspl{cnn} and are responsible for the majority of computations performed. As such they are a prime target for optimization. Take the following simplified formulation of the forward pass for example:
%
\begin{equation}
	y = x * w \qquad x,y \in \mathbb{R}^{N\times N} \quad w \in \mathbb{R}^{U\times U}
\end{equation}
%
The dimensions of the input and output tensor $x,y$ are generally much bigger than those of the weights $w$. In real world networks, we find $U=1,3,5$ for the weights and $N>100$ for the input and output. In simple terms, this is a convolution of a big tensor ($x$) with a small tensor ($w$), producing a big tensor ($y$). A dedicated hardware accelerator can make use of this by keeping the weights in a local memory and streaming the large image data in and out. Optimizations such as the Winograd and Fast Fourier Transform can help further reduce the computational footprint.

In contrast, during the backward pass we have to compute the following two convolutions, the first for the chain rule and the second for the gradient:
%
\begin{align}
	\Delta x &= \Delta y * \operatorname{flip}(w)  \label{eq:conv:chain} \\
	\Delta w &= x * \Delta y  \label{eq:conv:grad}
\end{align}
%
Note that $\operatorname{flip}(w)$ is $w$ rotated by $180^\circ$. The convolution in \eqnref{eq:conv:grad} has a completely different shape than the previous two: a big tensor ($x$) convolved with a big tensor ($\Delta y$), producing a small tensor ($w$).

\subsubsection{Striding}
\label{sec:compat:cnn:stride}

Strided convolutions and pooling operations are a common scheme to implement spatial down-sampling. A stride greater than one implies that not all values in the input tensor contribute equally to the output tensor. While not a problem for the forward pass, the operations in the backward pass become less regular since each incoming gradient may affect a different number of outgoing gradients. Subdividing the values into different cases produces regular sub-problems that can be treated independently. Strided convolutions for example can be decomposed into multiple unstrided convolutions.

\subsubsection{Non-linear Layers}
\label{sec:compat:cnn:nonlinear}

The ReLU activation function and max pooling are two prominent examples of non-linear layers commonly employed in DNNs. Implementation is trivial for the forward pass, since both operations boil down to determining the maximum over a set of numbers. During the backward pass however, implementation becomes more involved. ReLU needs to conditionally propagate the incoming gradients based on the corresponding values in the forward pass input. Max pooling is more complicated, as each of the gradients has multiple potential destinations in the pooling window. Additionally, multiple gradients may be propagated to the same location, essentially requiring the concept of an additive scattering operation for the backward pass.

\subsubsection{Layer Fusion}
\label{sec:compat:cnn:fusion}

Layers in \glspl{cnn} are generally followed by an element-wise activation function and/or a sub-sampling operation. Accelerators that only perform the forward pass can easily fuse these with the computation of the convolution. For training however, the inputs to each function must be preserved for the backward pass, thus rendering layer fusion impossible.



% ------------------------------------------------------------------------------
\subsection{Recurrent Neural Networks}
\label{sec:compat:rnn}

\glspl{rnn} generally consist of matrix-vector multiplications and activation function evaluations \cite{Goodfellow2016}. The former are BLAS2 operations that tend to be memory-bound, which is problematic. By processing multiple samples in parallel (i.e. introducing a batch size), these operations become matrix-matrix multiplications, thus falling under the BLAS3 category \cite{appleyard2016optimizing}. The same applies to \glspl{mlp} as well. Variations such as \gls{lstm} and \gls{gru} introduce additional bypass operations to compensate the ``Vanishing Gradient'' effect \cite{hochreiter2001gradient} during training, but the underlying structure remains the same. \glspl{rnn} have received little attention in terms of hardware acceleration, especially with respect to training. Our architecture fully supports training \glspl{lstm} and \glspl{gru}.



% ------------------------------------------------------------------------------
\subsection{Compression and Sparsity}
\label{sec:compat:zip}

Aggressive exploitation of sparsity is becoming more common for inference. Recent work has investigated the possibility to reduce the size of neural networks through quantization and compression \cite{Han2015}, as well as joint training and pruning \cite{han2015learning} techniques, while maintaining the network's accuracy. These approaches do not generally apply to training, and our architecture has no direct support for them.


==> tables/compat_layers.tex <==
\begin{table}
\begin{threeparttable}
\caption{Overview of the layers found in the \glspl{dnn} considered in this work, and hardware support in this work and \cite{azarkhish2017neurostream} for performing a full training step inside the \gls{hmc}.}
\label{tbl:compat:layers}
\newcommand{\LY}{\checkmark}
\newcommand{\LN}{--}
\newcommand{\NFB}{$\rightleftarrows$}
\newcommand{\NF}{$\rightarrow$}
\newcommand{\NB}{$\leftarrow$}
\newcommand{\NN}{--}
\begin{tabularx}{\linewidth}{@{}X ccccccccc@{}}
\toprule
    & \rotatebox{90}{Conv.}
    & \rotatebox{90}{Linear}
    & \rotatebox{90}{Max Pool}
    & \rotatebox{90}{Avg Pool}
    & \rotatebox{90}{Softmax}
    & \rotatebox{90}{ReLU}
    & \rotatebox{90}{Tanh/Sig}
    & \rotatebox{90}{Norm.\tnote{\ddag}}
    & \rotatebox{90}{Dropout} \\
\midrule
    \multicolumn{8}{@{}l@{}}{\textbf{Neural Networks}} \\
    AlexNet \cite{Krizhevsky2012}         & \LY & \LY & \LY & \LN & \LY & \LY & \LN & \LY & \LN \\ % conv, maxpool, linear, softmax, lrn, relu
    VGG 11/16/19 \cite{Simonyan2014}      & \LY & \LY & \LY & \LN & \LY & \LY & \LN & \LY & \LN \\ % conv, maxpool, linear, softmax, lrn, relu
    GoogLeNet \cite{Szegedy2015}          & \LY & \LY & \LY & \LY & \LY & \LY & \LN & \LY & \LY \\ % conv, maxpool, avgpool, linear, dropout, softmax, lrn, relu
    ResNet 18-152 \cite{he2016deep}       & \LY & \LY & \LY & \LY & \LY & \LY & \LN & \LN & \LN \\ % conv, maxpool, avgpool, linear, softmax, relu
    Incep. v2/v3 \cite{Szegedy2016}       & \LY & \LY & \LY & \LY & \LY & \LY & \LN & \LY & \LN \\ % conv, maxpool, avgpool, linear, softmax, relu
    Incep. v4 \cite{szegedy2017inception} & \LY & \LY & \LY & \LY & \LY & \LY & \LN & \LY & \LY \\ % conv, maxpool, avgpool, linear, dropout, softmax, relu
    RNNs/LSTMs \cite{Goodfellow2016}      & \LN & \LY & \LN & \LN & \LY & \LY & \LY & \LN & \LY \\
\midrule
    \multicolumn{8}{@{}l@{}}{\textbf{Hardware Support for Training}} \\
    NS \cite{azarkhish2017neurostream}               & \LN\tnote{*} & \LN\tnote{*} & \LN\tnote{\dag} & \LN\tnote{*} & \LY\tnote{\S} & \LN\tnote{\dag} & \LY\tnote{\S} & \LY\tnote{\S} & \LN \\
    NTX (this work)                       & \LY            & \LY            & \LY             & \LY & \LY\tnote{\S} & \LY             & \LY\tnote{\S} & \LY\tnote{\S} & \LY \\
\bottomrule
\end{tabularx}
\begin{tablenotes}
    \item[\dag] Only forward pass supported
    \item[\ddag] Local response and batch normalization
    \item[*] Requires expensive re-tiling of data
    \item[\S] div, exp, log, sqrt require iterative evaluation (see \secref{sec:progmod_exp})
\end{tablenotes}
\end{threeparttable}
\end{table}

